Transformer based Multilingual document Embedding model

One of the current state-of-the-art multilingual document embedding model LASER is based on the bidirectional LSTM neural machine translation model. This paper presents a transformer-based sentence/document embedding model, T-LASER, which makes three significant improvements. Firstly, the BiLSTM layers is replaced by the attention-based transformer layers, which is more capable of learning sequential patterns in longer texts. Secondly, due to the absence of recurrence, T-LASER enables faster parallel computations in the encoder to generate the text embedding. Thirdly, we augment the NMT translation loss function with an additional novel distance constraint loss. This distance constraint loss would further bring the embeddings of parallel sentences close together in the vector space; we call the T-LASER model trained with distance constraint, cT-LASER. Our cT-LASER model significantly outperforms both BiLSTM-based LASER and the simpler transformer-based T-LASER.

==> acknowledge.tex <==
\section{Acknowledgements}
The work described in this paper was supported by the Research Grants Council of the Hong Kong Special Administrative Region, China (Project Nos.  HKUST16200118 and T45-407/19N-1).

==> discussion.tex <==
\subsection{Discussion on the Effectiveness of Distance Constraint Training}



%\begin{figure*}
%   \vspace{-1.2cm}
%   \begin{center}
%     \begin{tabular}[t]{cc}
%       \hspace*{-5.00em}
%       \subfigure[\cnvsumen ; \cnvsumde ]{\includegraphics[width=.29\textwidth]{a500.png}} 
%       \hspace*{-2.9em}
%       &
%       \subfigure[\nvsumen; \nvsumde ]{\includegraphics[width=.29\textwidth]{b500.png}}
%       \hspace*{-2.em}
     
%       \subfigure[\cnvsumen ; \cnvsumde ]{\includegraphics[width=.29\textwidth]{a500bi.png}}
%       \hspace*{-2em}
       
%       \subfigure[\nvsumen ; \nvsumde ]{\includegraphics[width=.29\textwidth]{b500bi.png}}
       
       %\subfigure[cNTDV]{\resizebox{0.27\textwidth}{!}{\includegraphics{a500bi.png}}} 
       %\subfigure[NTDV ]{\resizebox{0.27\textwidth}{!}{\includegraphics{b500bi.png}}} 
%     \end{tabular}
%   \end{center}
%    \vspace{-0.6cm}
%    \caption{The distribution of embeddings from the four document classes (subfigure a, b) and the distribution of English and German embeddings (subfigure c, d) in the test set. }
%    \vspace{0.2cm}
%    \label{fig:dist_pair500}
%\end{figure*}




%We also explore the effectiveness of distance constraint training in previous studies. Here we adopt a GRUs based NMT framework as in [ref] and name it as NV model. 

The effectiveness of distance constraint training has also been illustrated vividly by a study from \cite{li2020}. NV \shortcite{li2020} in Fig. \ref{fig:dist_pair50}  is a gated recurrent units (GRUs) based document embedding models model, which has many similarities with LASER and T-LASER. However, the NV model does not have pivot target languages and uniformed dictionary as in LASER. Thus it has to rely solely on distance constraint loss to bridge the gap between parallel sentences. cNV is NV model trained with distance constraint loss in addition to the translation loss.

%Instead, it would use independent GRU encoder at the first layer, shared GRU encoder as the second layer, a unique dictionary for each language. cNV is NV model trained with distance constraint loss in addition to the translation loss.


\begin{figure*}[tbhp]
\vspace{-3mm}
   \begin{center}
     \begin{tabular}[t]{cc}
       \subfigure[%With distance constraint training 
       \cnvsumen ; \cnvsumde]{\resizebox{0.40\textwidth}{!}{\includegraphics{a50.PNG}}} &
       
       \subfigure[%Without  distance constraint training 
       \nvsumen ; \nvsumde]{\resizebox{0.40\textwidth}{!}{\includegraphics{b50.PNG}}} 
     \end{tabular}
   \end{center}
    \vspace{-0.6cm}
    \caption{ Embedding of 50 randomly sampled German documents (-) and their English translation (+) \cite{li2020}. NV is NMT based document embedding model. cNV is NV model trained with distance constraint loss in addition to the translation loss.}
    %\vspace{0.2cm}
    \vspace{0.5cm}
    \label{fig:dist_pair50}
\end{figure*}

Fig. \ref{fig:dist_pair50} sampled 50 German document from the RCV1/RCV2 dataset and shows the t-SNE projections of the embeddings of the original German document and their English translations. German documents are indicated by the positive sign, and its English translation is indicated by the negative sign. For example, the 4th German document is indicated by `-4'; its Engish translation is indicated by `+4'. The embedding on the left is obtained by cNV, while the embedding on the right is obtained by cNV. Clearly, cNV pairs the parallel documents closer to each other compared to the embedding from NV

%For example,the 2nd document German in the sampled set is indicated by `-2', whereas the English translation of the same document is indicated by `2'. It shows that when trained with distance constraint, the cNV model successfully projects the German and English embeddings into a pair, regardless of their different encoders and language inputs. On the other hand, NV cannot pair the English-German parallel document very well. 

 The results from this paper, in combination with study conducted by \cite{li2020} shows that shared layers in the NMT encoder alone a re insufficient to produce language-independent representation in the document embedding. To overcome this problem, we can either emulate the LASER setup, which includes pivots target language, shared encoder, and language-independent dictionary. We can also use a distant constraint loss term if one of the above conditions is not met, as illustrated by Fig. \ref{fig:dist_pair50}. From the result in \ref{tbl:cT-LASER}, we can also infer that combine these two approaches would accommodate each other and produce an even better result at a small cost of training speed.
 



%Therefore the translation loss would not drive the encoder to form shared embedding. We name document vector produced by the GRUs based NMT model as NV and the version trained with distance constraint as cNV.


%This also explains why the previous NV model must use an NMT as a bridge to achieve good classification performance, and why in the current cNV model the NMT is not necessary.


%Without the distance constraint, the English embedding and its corresponding German embedding of the same document is not guaranteed to lie in the same vector space and cannot be compared. To further illustrate this, we visualize the document embeddings of different languages using their t-SNE projections in Fig. \ref{fig:dist_pair500} and \ref{fig:dist_pair50}.
%Fig. \ref{fig:dist_pair500} shows the NV/cNV embeddings of German documents in the ${en\rightarrow de}$ test set. We also translate the same documents into a mirrored English set with the NMT to show the distribution of the same documents in a different language. 
%In  Fig. \ref{fig:dist_pair500} (a) and (b), the 4 types of documents are plotted in 4 different colors (red: Corporate/Industrial, blue: Economics, green: Government/Social, yellow: Market). The document embeddings are clearly divided into 4 clusters, but only when they are trained with distance constraint then their German embeddings and English embeddings (from the translation of the German texts) are indistinguishable if they belong to the same type. On the other hand, in Fig. \ref{fig:dist_pair500} (c) and (d), English embeddings are shown in red while their German counterparts of the same documents are shown in green regardless of their document types.
%It is clear that without the distance constraint training, the NV document embeddings are segregated by the languages into two major clusters.

%These figures show that simply sharing layers in the NV model without distance constraint training is not sufficient to produce similar embeddings from two languages and they cannot be compared.

